Input-to-state stability of infinite-dimensional systems: recent results and open questions

In a pedagogical but exhaustive manner, this survey reviews the main results on input-to-state stability (ISS) for infinite-dimensional systems. This property allows estimating the impact of inputs and initial conditions on both the intermediate values and the asymptotic bound on the solutions. ISS has unified the input-output and Lyapunov stability theories and is a crucial property in the stability theory of control systems as well as for many applications whose dynamics depend on parameters, unknown perturbations, or other inputs. In this paper, starting from classic results for nonlinear ordinary differential equations, we motivate the study of ISS property for distributed parameter systems. Then fundamental properties are given, as an ISS superposition theorem and characterizations of (global and local) ISS in terms of Lyapunov functions. We explain in detail the functional-analytic approach to ISS theory of linear systems with unbounded input operators, with special attention devoted to ISS theory of boundary control systems. The Lyapunov method is shown to be very useful for both linear and nonlinear models, including parabolic and hyperbolic partial differential equations. Next, we show the efficiency of the ISS framework to study the stability of large-scale networks, coupled either via the boundary or via the interior of the spatial domain. ISS methodology allows reducing the stability analysis of complex networks, by considering the stability properties of its components and the interconnection structure between the subsystems. An extra section is devoted to ISS theory of time-delay systems with the emphasis on techniques, which are particularly suited for this class of systems. Finally, numerous applications are considered in this survey, where ISS properties play a crucial role in their study. This survey suggests many open problems throughout the paper.

==> Figure_Characterizations.tex <==
\begin{figure*}[tbh]
\centering
\begin{tikzpicture}[>=implies,thick]
%\node (Unif_Level) at (-4,5.5) {Uniform GAS level};
%\node (Nonunif_Level) at (-4.25, 2.5) {Non-uniform GAS level};

\node (ISS) at (-0.5,0.4) {ISS};
\node (UAG) at (-2.7,0.4) {UAG};

%\node (WURS) at  (3.5,-0.5)  {WURS};
%\node (WURSLF) at (7,0.4) {$\exists$ WURS-LF};
%\node (ISSLF) at (3,0.4) {\color{blue} $\exists$ ISS-LF};

\draw [rounded corners] (-8.4,1.2) rectangle (-0.2,0.1);
\node (Thm5) at (-4.4,0.9) {\footnotesize Theorem~\ref{thm:UAG_equals_ULIM_plus_LS}};

%\node (Thm6) at (-8.75,-0.1) {\footnotesize \color{blue} Theorem~\ref{thm:MainResult_Characterization_ISS_EQ_Banach_Spaces}};
%\node (Thm3) at (1.05,0.9) {\footnotesize \color{blue} Theorem~\ref{thm:Characterization_ISS}};

 \node (Thm8) at (-3.2,-1) {\footnotesize Theorem~\ref{wISS_equals_sAG_GS}};

 %\node (Thm2) at (4.6,-2.38) {\footnotesize \color{blue} Theorem~\ref{Characterization_LISS}};

\node (Rem) at (-4,-2.35) {\footnotesize Remark~\ref{rem:LIMAG}};


\draw [rounded corners] (-6.4,-1.8) rectangle (-0.2,-0.7);

\draw[thick,double equal sign distance,<->] (ISS) to (UAG);
%\draw[thick,double equal sign distance,->] (ISS) to (WURS);
%\draw[thick,double equal sign distance,->] (WURS) to (WURSLF);
%\draw[thick,double equal sign distance,->] (WURSLF) to (ISSLF);
%\draw[thick,double equal sign distance, blue,dashed,<->] (ISSLF) to (ISS);

\node (ULIM_UGS) at (-4.7,0.4) {ULIM$\,\wedge\,$UGS};
\node (ULIM_ULS) at (-7.4,0.4) {ULIM$\,\wedge\,$ULS};
%\node (ULIM_0ULS)at (-10.2,0.4) {\color{blue} ULIM$\,\wedge\,$0-ULS};
 
\draw[thick,double equal sign distance,<->] (ULIM_UGS) to (UAG);
\draw[thick,double equal sign distance,<->] (ULIM_ULS) to (ULIM_UGS);
%\draw[thick,double equal sign distance,blue,dashed,<->] (ULIM_0ULS) to (ULIM_ULS);

\node (sISS) at (-0.6,-1.5) {sISS};
\node (sAG_UGS) at (-2.7,-1.5) {sAG$\,\wedge\,$UGS};
\node (sLIM_UGS) at (-5.4,-1.5) {sLIM$\,\wedge\,$UGS};
\draw[<->,double equal sign distance] (sISS) to (sAG_UGS);

\draw[<->,double equal sign distance] (sLIM_UGS) to (sAG_UGS);

\draw[thick,double equal sign distance,->] (-3.3,0) to (-3.3,-0.6);
\draw[red,double equal sign distance,->,degil]  (-2.95,-0.6) to (-2.95,0);
\node[red] (notImp_ix) at (-2.45,-0.3) {\footnotesize(ix)};


\draw[red,double equal sign distance,->,degil]  (0.9,-2.45) to (0.2,-2.45);
\node[red] (vi) at (1.3,-2.45) {\footnotesize(vi)};

\draw[red,double equal sign distance,<-,degil]  (0.9,-2.95) to (0.2,-2.95);
\node[red] (vii) at (1.3,-2.95) {\footnotesize(vii)};

\draw[red,double equal sign distance,->,degil]  (0.9,-1.3) to (0.2,-1.3);
\node[red] (iv) at (1.3,-1.3) {\footnotesize(iv)};

\draw[red,double equal sign distance,<-,degil]  (0.9,-1.7) to (0.2,-1.7);
\node[red] (v) at (1.3,-1.7) {\footnotesize(v)};


%\node[red] (notImp51) at (1,-2.45) { $\not\Leftarrow$\,(vi)};
% \node[red] (notImp52) at (1,-2.95) { $\not\Rightarrow$\,(vii)};
%\node[red] (notImp61) at (1,-1.7) { $\not\Rightarrow$\,(v)};
%\node[red] (notImp62) at (1,-1.3) { $\not\Leftarrow$\,(iv)};


%\node[double equal sign distance,red,rotate=50](NonConv3) at (0.9,-0.6) {$\not\Uparrow$};
%\node[red] (notImp_new) at (0.4,-0.6) {(iii) };

\node (AG_UGS) at (-2.7,-2.75) {AG$\,\wedge\,$UGS};
\node (LIM_UGS) at (-5.4,-2.75) {LIM$\,\wedge\,$UGS};
%\node (LIM_pGS_ULS) at (-5,-3.5) {LIM$\,\wedge\,$pGS$\,\wedge\,$ULS};

\node (AG_ULS) at (-2.7,-3.9) {AG$\,\wedge\,$ULS};
%\node (LIM_ULS) at (-2,-4.5) {LIM$\,\wedge\,$ULS};


\node (AG_0UGAS) at (3.1,-1.5) {AG$\,\wedge\,$0-UGAS};
%\node (AG_LISS) at (5.8,-2.75) {\color{blue}AG$\,\wedge\,$LISS};
\node (AG_0UAS) at (3.1,-2.75) {AG$\,\wedge\,$0-UAS};
\node (AG_0LS) at (3.1,-3.9) {AG$\,\wedge\,$0-ULS};
\node (AG_0GAS) at (5.8,-3.9) {AG$\,\wedge\,$0-GAS};

%\node (LIM_0LS) at (3.5,-4.5) {LIM$\,\wedge\,$0-ULS};
%\node (LIM_0GAS) at (7,-4.5) {LIM$\,\wedge\,$0-GAS};



%Relations AG_UGS and AG_ULS
\draw[double equal sign distance,->]  ($(AG_UGS)+(-0.2,-0.3)$) to ($(AG_ULS)+(-0.2,0.3)$);
\draw[red,double equal sign distance,<-,degil]  ($(AG_UGS)+(0.2,-0.3)$) to ($(AG_ULS)+(0.2,0.3)$);
\node[red] (viii) at ($\weight*(AG_ULS)+\weight*(AG_UGS) + (0.75,0)$) {\footnotesize(viii)};


%Relations AG_0UGAS and AG_0UAS
\draw[double equal sign distance,->]  ($(AG_0UGAS)+(-0.2,-0.3)$) to ($(AG_0UAS)+(-0.2,0.3)$);
\draw[red,double equal sign distance,<-,degil]  ($(AG_0UGAS)+(0.2,-0.3)$) to ($(AG_0UAS)+(0.2,0.3)$);
\node[red] (ii) at ($\weight*(AG_0UAS)+\weight*(AG_0UGAS) + (0.6,0)$) {\footnotesize(ii)};

%Relations AG_0UAS and AG_0LS
\draw[double equal sign distance,->]  ($(AG_0UAS)+(-0.2,-0.3)$) to ($(AG_0LS)+(-0.2,0.3)$);
\draw[red,double equal sign distance,<-,degil]  ($(AG_0UAS)+(0.2,-0.3)$) to ($(AG_0LS)+(0.2,0.3)$);
\node[red] (i) at ($\weight*(AG_0LS)+\weight*(AG_0UAS) + (0.6,0)$) {\footnotesize(i)};

% \draw[red,double equal sign distance,<-,degil]  ($(AG_0UAS)+(0.2,-0.3)$) to ($(AG_0LS)+(0.2,0.3)$);
% 
% \node[red] (i) at ($\weight*(AG_0LS)+\weight*(AG_0UAS) + (0.7,0)$) {\footnotesize(i)};

\coordinate (ISS_1) at ($(ISS) + (-0.5,0)$);
\coordinate (AG_0UGAS_1) at ($(AG_0UGAS) + (-0.5,0)$);
\coordinate (coord1) at ($\third*(ISS_1)+\twothirds*(AG_0UGAS_1)$);
\coordinate (coord2) at ($\twothirds*(ISS_1)+\third*(AG_0UGAS_1)$);

\draw[red,double equal sign distance,->,degil]  (coord1) to (coord2);
\node[red] (iii) at ($\weight*(ISS_1) + \weight*(AG_0UGAS_1) + (-0.45,-0.15)$) {\footnotesize(iii)};




\draw[thick,double equal sign distance,->] ($(sAG_UGS)+(-0.2,-0.37)$) to ($(AG_UGS)+(-0.2,0.27)$);

  \coordinate (A2) at ($(sAG_UGS)+(0.2,-0.37)$);
  \coordinate (B2) at ($(AG_UGS)+(0.2,0.27)$);
%\path (B2) -- node (Q2) {\footnotesize\color{red}{???}} (A2);
  %\coordinate (QQ2) at ($(Q2)+(0,-0.2)$);
 %\draw[thick,double equal sign distance,->] (B2) -- (QQ2) -- (A2);
\node[red] (Quest) at (-2.5,-2.23) {\footnotesize ???};
\draw[double equal sign distance,-] (B2) to ($(B2)+(0,0.09)$);
\draw[double equal sign distance,->] ($(B2)+(0,0.42)$) to (A2);

\draw[double equal sign distance,->]  ($(AG_UGS)+(-0.2,-0.3)$) to ($(AG_ULS)+(-0.2,0.3)$);

\draw[thick,double equal sign distance,<->] (AG_UGS) to (LIM_UGS);
%\draw[thick,double equal sign distance,<->] (AG_UGS) to  (LIM_pGS_ULS);

\draw[thick,double equal sign distance,->] (ISS) to (AG_0UGAS);
%\draw[thick,double equal sign distance,blue,dashed,<->]  (AG_LISS) to (AG_0UAS);

%\draw[thick,double equal sign distance,->]  (AG_0UAS) to (AG_0LS);
\draw[thick,double equal sign distance,<->]  (AG_0LS) to (AG_0GAS);
%\draw[thick,double equal sign distance,->]  (AG_0LS) to (LIM_0LS);

\draw[thick,double equal sign distance,->] ($(AG_ULS)+(0.9,-0.12)$)  to ($(AG_0LS)+(-1.1,-0.12)$);

  \coordinate (A1) at ($(AG_ULS)+(0.9,0.12)$);
  \coordinate (B1) at ($(AG_0LS)+(-1.1,0.12)$);
\path (B1) -- node (Q) {\footnotesize\color{red}{???}} (A1);
    \draw[thick,double equal sign distance,->] (B1) -- (Q) -- (A1);
%\draw[thick,double equal sign distance,<-] (A1)  -- (B1) node[midway,fill=white] {\footnotesize{\color{red}???}};
%\node[red] (Quest5) at (0,-3.6) {\footnotesize ???};


%\draw[thick,double equal sign distance,->]  (LIM_ULS) to (LIM_0LS);

%\draw[thick,double equal sign distance,<->]  (LIM_0LS) to (LIM_0GAS);
\end{tikzpicture}
%\caption[caption]{Relations between stability notions for infinite-dimensional control systems, satisfying REP and BRS properties:
\caption[caption]{Relations between stability properties of
  infinite-dimensional systems, which have a robust equilibrium point and
  bounded reachability sets:
\begin{itemize}%[leftmargin=5mm]
\setlength{\itemindent}{5mm}
   \item Black arrows show implications or equivalences which hold for general control systems
in infinite dimensions.
\item {\color{red}Red arrows (with the negation sign)}
are implications which do not hold, due to the counterexamples
presented in this paper (see Remark~\ref{rem:Nonimplications}).
%\item {\color{blue}Blue dashed equivalences} are proved only for systems of the form \eqref{InfiniteDim} and under certain additional conditions.
\item Black arrows with question marks inside mean that it is not known right now (as far as the authors are concerned), whether the converse implications hold or not.
\end{itemize}
}
\label{fig:ISS_Equiv_Evolution_Equations}
\end{figure*}




==> sec_Conventions.tex <==

\section{Conventions}

%This is a Fabian's list, a bit extended and edited by Andrii.

{\bf General}

\begin{itemize}
  %\item How do we organize file sharing?
	\item Every section should be written in a separate tex file
	%\item There is a conditional operator "ifAndo". Currently it is set to Andofalse.
\end{itemize}


{\bf Symbols}

\begin{itemize}
  %\item A full list of symbols which are used in the book will be called "Glossary", and will be put to the end of the book. 
  %\item If anybody is adding a new symbol, he/she should send an email to everybody telling this.
  %\item $C(X,U)$ should be $C_b(X,U)$
	\item We use semicolons in the definitions of sets.
	\item We use always $\overline{\lim}$ instead of $\limsup$.
\end{itemize}

{\bf Typesetting}

\begin{itemize}
	%\item AM: I propose to use regularly "stackrel" in the derivations of the formulas. This saves a lot of time for the readers.
  \item No acronyms in section titles. Section titles are not capitalized. 
  \item Commas and periods appear at the end of displayed formulas.
  \item New notions in definitions should be emphasized via \emph{$\backslash$ emph}.
  \item No other fonts are used for emphasizing.
  
 \item formulas in sections are numbered by two numbers (section number. subsection number). 
 \item Theorems with numbers and the like are capitalized.  (as in Theorem
   3.14, Figure 3.6). Figure is spelled out. Other uses of theorem and lemma are not capitalized.
 \item Theorems, lemmas, definitions and all other environments are numbered consecutively with just one uniform counter.
 \item There are no bulleted lists in theorems, definitions etc (we need numbers in order to make each item citable). Bulleted lists are strictly limited to informal discussions.
 \item Lists in theorems etc. are numbered with small roman numbers.
 \item There are no boxed formulas. We box the most important theorems in each chapter (possibly with the exception of the background chapters?)
 %\item Remarks are set in roman font and are contained in a latex environment called remark. This is taken care of in the master file. Nothing special needs to be done in the remarks.
 \item Definitions, remarks and examples carry an end-symbol. This can be created by using the
   command \verb"\ersymbol".
  \item Examples are written in roman font.
 \item For assumptions a latex environment called assumption is used.
 \item Proofs are written in the proof environment.
 \item we write $i$th, not $i^{th}$, nor $i$-th.
 \item sign functions ($\mathrm {sgn}$) , and also $\cos,\sin$ etc are set in roman font.
\end{itemize}

{\bf Language}

\begin{itemize}
  \item The paper is written in American English.
  %\item new acronyms are avoided, unless there is a really strong case for them.
  %\item we try to be as English as possible, so formulations like ``The
    %differentiability of absolutely continuous functions in a.e. sense''
    %(which Andrii likes) are avoided.
  %\item we say ``locally Lipschitz continuous'' not ``Lipschitz continuous
    %on bounded sets''.
  %\item we avoid ``w.r.t.'' (mostly it can be said more elegantly in
    %another way)
  %\item we avoid ``s.t.'' in text (see for example end of p.13) 
\end{itemize}


{\bf Figures}

\begin{itemize}
  \item Figures are produced in black and white, no color unless strictly necessary.
  %\item On Dropbox or alternative we keep a folder ``Matlab'' where all Matlab scripts are placed that are required to produce figures
  %\item Matlab figures are always transformed to tikz-figures. Fabian knows how to do this and can help.
  \item Periods at the end of captions
\end{itemize}

{\bf References}

\begin{itemize}
  \item Referencing to other sections is done by explicit reference to a
    label. We avoid the use of ``in previous chapters'', ``in the previous
    section''. ``The previous equation'', ``the previous theorem'' are
    fine, if this is really used shortly after the item in question.
  \item Where possible, names of authors are given as on the cited
    material, in particular with or without 2nd initial, as the case may be.
  \item journal titles are not abbreviated 
  \item acronym short names of journal titles are not mentioned (so not
    IEEE/ACM Transactions on Networking (TON)).
  \item  journal names are stated as in the official journal name

%e.g. it would IEEE Transaction on Automatic Control, and not what google
%scholar frequently suggests ``Automatic Control, IEEE Transactions on''

\item  all entries need, pages, locations or address of publisher, etc.

\item  book titles are capitalized

\item  we do not cite documents from sources that explicitly say that the documents are not to be cited

\item  when there is a preliminary technical report we try to cite the refereed version instead

\item  papers appearing in CDC are cited as

... in Proc. (number)th IEEE Conference on Decision and Control, location, pages, year.

Similar rules for other conferences. 

\item In the bibtex file for conference entries, location is a separate
  item. Location is not included in the booktitle.
\end{itemize}

{\bf Index}
\begin{itemize}
  \item We  aim for redundancy.
  \item Where useful we have a separate index entry for the definition of
    a concept.
\end{itemize}

%\newpage

{\bf List of symbols}

\begin{itemize}
  \item state variables are denoted by lower case letters ($x_i$ etc.) 
\item Matrices are not set in bold.
%\item Whenever we have a constant that bounds a quantity, as in (3.1). It is called $C$ with a suggestive index. E.g. in (3.1) use $C_p$.
  \item Fixed points are denoted by superscript $^*$ as in $x^*$
\end{itemize}



{\bf Notations for inputs, disturbances and controls}

\begin{itemize}
  \item $d$ is always a disturbance, which does not induce asymptotic gains.
  \item $u$ is always an input (or: disturbance input), which induces asymptotic gains.
  %\item In all Chapters on ISS applications $u$ is always a control (or: control input).
	%The disturbances acting on the system (which induce some asymptotic gains) are called $w$.
	%In particular, the ISS stabilization is then a designing a feedback controller $u$ so that the system is ISS w.r.t. the acting disturbances $w$.
\end{itemize}


{\bf Notations for comparison functions}

\begin{itemize}
  \item $\beta$ is a $\KL$-function, showing the transient behavior in the definitions of ISS, ISDS, etc.
  \item An ISS gain is always called $\gamma$
  \item An ISS Lyapunov gain is always called $\chi$
  \item The upper and lower bounds for Lyapunov functions in the definition of a Lyapunov function are always $\psi_1,\psi_2$
  \item The decay (dissipation) rate in the definition of an ISS Lyapunov function is always called $\alpha$.
\end{itemize}





